Fixed product preserving mappings on Banach algebras

In this paper, we describe linear maps between complex Banach algebras that preserve products equal to fixed elements. This generalizes some important special cases where the fixed elements are the zero or identity element. First we show that if such map preserves products equal to a finite-rank operator, then it must also preserve the zero product. In several instances, this is enough to show that a product preserving map must be a scalar multiple of an algebra homomorphism. Second, we explore a more general problem concerning the existence of product preserving maps and the relationship between the fixed elements. Lastly, motivated by Kaplansky's problem on invertibility preservers, we show that maps preserving products equal to fixed invertible elements are either homomorphisms or antihomomorphisms multiplied on the left by a fixed element.

==> bib.tex <==
@article {watkins,
    AUTHOR = {Watkins, W.},
     TITLE = {Linear maps that preserve commuting pairs of matrices},
   JOURNAL = {Linear Algebra Appl.},
  FJOURNAL = {Linear Algebra and its Applications},
    VOLUME = {14},
      YEAR = {1976},
    NUMBER = {1},
     PAGES = {29--35},
      ISSN = {0024-3795},
   MRCLASS = {15A27},
  MRNUMBER = {480574},
MRREVIEWER = {M. Shafqat Ali},
       DOI = {10.1016/0024-3795(76)90060-4},
       URL = {https://doi.org/10.1016/0024-3795(76)90060-4},
}

@book{cohn,
  title={Further algebra and applications},
  author={Cohn, P. M.},
  year={2002},
  publisher={Springer Science \& Business Media}
}

@book{kaplanskyinv,
  title={Algebraic and analytic aspects of operator algebras},
  author={Kaplansky, I.},
  volume={1},
  year={1970},
  publisher={American Mathematical Soc.}
}

@article{costaraproducts,
  title={Linear bijective maps preserving fixed products of matrices},
  author={Costara, C.},
  journal={J. Algebra},
  volume={587},
  pages={336--343},
  year={2021},
  publisher={Elsevier}
}

@article{rieffel,
  title={Dimension and Stable Rank in the {K}-Theory of {C}*-Algebras},
  author={Rieffel, M. A.},
  journal={Proc. London Math. Soc.},
  volume={3},
  number={2},
  pages={301--333},
  year={1983},
  publisher={Wiley Online Library}
}

@article {lin,
    AUTHOR = {Lin, Y.-F.},
     TITLE = {Commutativity-preserving maps on {L}ie ideals of prime
              algebras},
   JOURNAL = {Linear Algebra Appl.},
  FJOURNAL = {Linear Algebra and its Applications},
    VOLUME = {371},
      YEAR = {2003},
     PAGES = {361--368},
      ISSN = {0024-3795},
   MRCLASS = {17B99},
  MRNUMBER = {1997381},
MRREVIEWER = {Yu Cai Su},
       DOI = {10.1016/S0024-3795(03)00484-1},
       URL = {https://doi.org/10.1016/S0024-3795(03)00484-1},
}

@article {bottapiercewatkins,
    AUTHOR = {Botta, P. and Pierce, S. and Watkins, W.},
     TITLE = {Linear transformations that preserve the nilpotent matrices},
   JOURNAL = {Pacific J. Math.},
  FJOURNAL = {Pacific Journal of Mathematics},
    VOLUME = {104},
      YEAR = {1983},
    NUMBER = {1},
     PAGES = {39--46},
      ISSN = {0030-8730},
   MRCLASS = {15A23 (20G15)},
  MRNUMBER = {683726},
MRREVIEWER = {Marvin Marcus},
       URL = {http://projecteuclid.org/euclid.pjm/1102723816},
}

@article {piercewatkins,
    AUTHOR = {Pierce, S. and Watkins, W.},
     TITLE = {Invariants of linear maps on matrix algebras},
   JOURNAL = {Linear and Multilinear Algebra},
  FJOURNAL = {Linear and Multilinear Algebra},
    VOLUME = {6},
      YEAR = {1978/79},
    NUMBER = {3},
     PAGES = {185--200},
      ISSN = {0308-1087},
   MRCLASS = {15A27},
  MRNUMBER = {512994},
MRREVIEWER = {W. S. Martindale, III},
       DOI = {10.1080/03081087808817237},
       URL = {https://doi.org/10.1080/03081087808817237},
}

@article {bresarsemrl,
    AUTHOR = {Bre\v{s}ar, M. and \v{S}emrl, P.},
     TITLE = {Mappings which preserve idempotents, local automorphisms, and
              local derivations},
   JOURNAL = {Canad. J. Math.},
  FJOURNAL = {Canadian Journal of Mathematics. Journal Canadien de
              Math\'{e}matiques},
    VOLUME = {45},
      YEAR = {1993},
    NUMBER = {3},
     PAGES = {483--496},
      ISSN = {0008-414X},
   MRCLASS = {47B47 (46H99 47D99)},
  MRNUMBER = {1222512},
MRREVIEWER = {A. R. Sourour},
       DOI = {10.4153/CJM-1993-025-4},
       URL = {https://doi.org/10.4153/CJM-1993-025-4}
}

@article {bresarsemrl2,
    AUTHOR = {Bre\v{s}ar, M. and \v{S}emrl, P.},
     TITLE = {On bilinear maps on matrices with applications to
              commutativity preservers},
   JOURNAL = {J. Algebra},
  FJOURNAL = {Journal of Algebra},
    VOLUME = {301},
      YEAR = {2006},
    NUMBER = {2},
     PAGES = {803--837},
      ISSN = {0021-8693},
   MRCLASS = {16S50},
  MRNUMBER = {2236769},
MRREVIEWER = {Leon Van Wyk},
       DOI = {10.1016/j.jalgebra.2005.11.002},
       URL = {https://doi.org/10.1016/j.jalgebra.2005.11.002},
}

@article {bresar,
    AUTHOR = {Bre\v{s}ar, M.},
     TITLE = {Commuting traces of biadditive mappings,
              commutativity-preserving mappings and {L}ie mappings},
   JOURNAL = {Trans. Amer. Math. Soc.},
  FJOURNAL = {Transactions of the American Mathematical Society},
    VOLUME = {335},
      YEAR = {1993},
    NUMBER = {2},
     PAGES = {525--546},
      ISSN = {0002-9947},
   MRCLASS = {16W25 (16N60 16W10)},
  MRNUMBER = {1069746},
MRREVIEWER = {Howard E. Bell},
       DOI = {10.2307/2154392},
       URL = {https://doi.org/10.2307/2154392},
}

@article {julius,
    AUTHOR = {Julius, H.},
     TITLE = {On maps sending rank-{$\kappa$} idempotents to idempotents},
   JOURNAL = {Oper. Matrices},
  FJOURNAL = {Operators and Matrices},
    VOLUME = {13},
      YEAR = {2019},
    NUMBER = {3},
     PAGES = {855--865},
      ISSN = {1846-3886},
   MRCLASS = {15A04},
  MRNUMBER = {4008517},
       DOI = {10.7153/oam-2019-13-61},
       URL = {https://doi.org/10.7153/oam-2019-13-61},
}

@article{alaminos,
  title={Maps preserving zero products},
  author={Alaminos, J. and Bre{\v{s}}ar, M. and Extremera, J. and Villena, A. R.},
  journal={Studia Math},
  volume={193},
  number={2},
  pages={131--159},
  year={2009}
}

@article{burgosmarquezgarciamoralescampoy,
  title={Determining {J}ordan (triple) homomorphisms by invertibility preserving conditions},
  author={Burgos, M. and M{\'a}rquez-Garc{\'\i}a, A.C. and Morales-Campoy, A.},
  journal={Linear Multilinear Algebra},
  volume={63},
  number={7},
  pages={1294--1308},
  year={2015},
  publisher={Taylor \& Francis}
}

@inproceedings{mbekhta,
  title={A {H}ua type theorem and linear preserver problems},
  author={Mbekhta, M.},
  booktitle={Math. Proc. R. Ir. Acad.},
  pages={109--121},
  year={2009},
  organization={JSTOR}
}

@article {litsing,
    AUTHOR = {Li, C.-K. and Tsing, N.-K.},
     TITLE = {Linear preserver problems: a brief introduction and some
              special techniques},
   JOURNAL = {Linear Algebra Appl.},
  FJOURNAL = {Linear Algebra and its Applications},
    VOLUME = {162/164},
      YEAR = {1992},
     PAGES = {217--235},
      ISSN = {0024-3795},
   MRCLASS = {15A04 (15A72)},
  MRNUMBER = {1148401},
MRREVIEWER = {William Watkins},
       DOI = {10.1016/0024-3795(92)90377-M},
       URL = {https://doi.org/10.1016/0024-3795(92)90377-M},
}

@article {catalanohsukapalko,
    AUTHOR = {Catalano, L. and Hsu, S. and Kapalko, R.},
     TITLE = {On maps preserving products of matrices},
   JOURNAL = {Linear Algebra Appl.},
  FJOURNAL = {Linear Algebra and its Applications},
    VOLUME = {563},
      YEAR = {2019},
     PAGES = {193--206},
      ISSN = {0024-3795},
   MRCLASS = {15A86 (16W10)},
  MRNUMBER = {3872987},
       DOI = {10.1016/j.laa.2018.10.029},
       URL = {https://doi.org/10.1016/j.laa.2018.10.029},
}

@article{costara,
  title={Linear bijective maps preserving fixed products of matrices},
  author={Costara, C.},
  journal={J. Algebra},
  fjournal={Journal of Algebra},
  year={2021},
  publisher={Elsevier}
}

@book{sinclair,
  title={Automatic continuity of linear operators},
  author={Sinclair, A. M.},
  volume={21},
  year={1976},
  publisher={Cambridge University Press}
}

@article{GJV,
title = "On maps preserving {L}ie products equal to a rank-one nilpotent",
journal = "Linear Algebra Appl.",
volume = "593",
pages = "212 - 227",
year = "2020",
issn = "0024-3795",
doi = "https://doi.org/10.1016/j.laa.2020.02.007",
url = "http://www.sciencedirect.com/science/article/pii/S0024379520300665",
author = "V. Ginsburg and H. Julius and R. Velasquez",
keywords = "Linear preservers, Commutativity preserving maps, Rank-one nilpotent",
abstract = "Let ϕ be a bijective linear map on the algebra of n×n complex matrices such that ϕ(e12)=e12 and [ϕ(A),ϕ(B)]=e12 whenever [A,B]=e12. The purpose of this paper is to describe ϕ. Surprisingly, ϕ has a different description from maps preserving zero Lie products."
}

@article {semrl,
    AUTHOR = {\v{S}emrl, P.},
     TITLE = {Linear mappings preserving square-zero matrices},
   JOURNAL = {Bull. Austral. Math. Soc.},
  FJOURNAL = {Bulletin of the Australian Mathematical Society},
    VOLUME = {48},
      YEAR = {1993},
    NUMBER = {3},
     PAGES = {365--370},
      ISSN = {0004-9727},
   MRCLASS = {15A04 (47B49)},
  MRNUMBER = {1248039},
MRREVIEWER = {Chi-Kwong Li},
       DOI = {10.1017/S0004972700015811},
       URL = {https://doi.org/10.1017/S0004972700015811},
}

@article {semrl2,
    AUTHOR = {\v{S}emrl, P.},
     TITLE = {Commutativity preserving maps},
   JOURNAL = {Linear Algebra Appl.},
  FJOURNAL = {Linear Algebra and its Applications},
    VOLUME = {429},
      YEAR = {2008},
    NUMBER = {5-6},
     PAGES = {1051--1070},
      ISSN = {0024-3795},
   MRCLASS = {16S50 (15A04 15A27 16W20 47B49 81Q10)},
  MRNUMBER = {2433163},
MRREVIEWER = {Tatjana Petek},
       DOI = {10.1016/j.laa.2007.05.006},
       URL = {https://doi.org/10.1016/j.laa.2007.05.006},
}

@article {chebotar,
    AUTHOR = {Chebotar, M. A. and Ke, W.-F. and Lee, P.-H. and Wong, N.-C.},
     TITLE = {Mappings preserving zero products},
   JOURNAL = {Studia Math.},
  FJOURNAL = {Studia Mathematica},
    VOLUME = {155},
      YEAR = {2003},
    NUMBER = {1},
     PAGES = {77--94},
      ISSN = {0039-3223},
   MRCLASS = {47B48 (16S99 46L05 46L10 46L30)},
  MRNUMBER = {1961162},
MRREVIEWER = {Lajos Moln\'{a}r},
       DOI = {10.4064/sm155-1-6},
       URL = {https://doi.org/10.4064/sm155-1-6},
}

@article {beasleypullman,
    AUTHOR = {Beasley, L. B. and Pullman, N. J.},
     TITLE = {Linear operators preserving idempotent matrices over fields},
   JOURNAL = {Linear Algebra Appl.},
  FJOURNAL = {Linear Algebra and its Applications},
    VOLUME = {146},
      YEAR = {1991},
     PAGES = {7--20},
      ISSN = {0024-3795},
   MRCLASS = {15A04},
  MRNUMBER = {1083460},
MRREVIEWER = {Donald W. Robinson},
       DOI = {10.1016/0024-3795(91)90016-P},
       URL = {https://doi.org/10.1016/0024-3795(91)90016-P},
}

@article {beasley,
    AUTHOR = {Beasley, L. B.},
     TITLE = {Linear transformations on matrices: {T}he invariance of rank
              {$k$} matrices},
   JOURNAL = {Linear Algebra Appl.},
  FJOURNAL = {Linear Algebra and its Applications},
    VOLUME = {3},
      YEAR = {1970},
     PAGES = {407--427},
      ISSN = {0024-3795},
   MRCLASS = {15.30},
  MRNUMBER = {271127},
MRREVIEWER = {Robert C. Thompson},
       DOI = {10.1016/0024-3795(70)90033-9},
       URL = {https://doi.org/10.1016/0024-3795(70)90033-9},
}

@article {omladic,
    AUTHOR = {Omladi\v{c}, M.},
     TITLE = {On operators preserving commutativity},
   JOURNAL = {J. Funct. Anal.},
  FJOURNAL = {Journal of Functional Analysis},
    VOLUME = {66},
      YEAR = {1986},
    NUMBER = {1},
     PAGES = {105--122},
      ISSN = {0022-1236},
   MRCLASS = {47B47 (47D99)},
  MRNUMBER = {829380},
MRREVIEWER = {A. R. Sourour},
       DOI = {10.1016/0022-1236(86)90084-4},
       URL = {https://doi.org/10.1016/0022-1236(86)90084-4},
}

@article {laffey,
    AUTHOR = {Laffey, T. J.},
     TITLE = {Simultaneous triangularization of matrices---low rank cases
              and the nonderogatory case},
   JOURNAL = {Linear Multilinear Algebra},
  FJOURNAL = {Linear and Multilinear Algebra},
    VOLUME = {6},
      YEAR = {1978/79},
    NUMBER = {4},
     PAGES = {269--305},
      ISSN = {0308-1087},
   MRCLASS = {15A21},
  MRNUMBER = {515915},
MRREVIEWER = {O. O. Romanovs\cprime ki\u{\i}},
       DOI = {10.1080/03081087808817249},
       URL = {https://doi.org/10.1080/03081087808817249},
}

@article {guralnick,
    AUTHOR = {Guralnick, R. M.},
     TITLE = {A note on pairs of matrices with rank one commutator},
   JOURNAL = {Linear and Multilinear Algebra},
  FJOURNAL = {Linear and Multilinear Algebra},
    VOLUME = {8},
      YEAR = {1979/80},
    NUMBER = {2},
     PAGES = {97--99},
      ISSN = {0308-1087},
   MRCLASS = {15A03},
  MRNUMBER = {552353},
MRREVIEWER = {C. F. Moppert},
       DOI = {10.1080/03081087908817305},
       URL = {https://doi.org/10.1080/03081087908817305},
}

@article {amitsurrowen,
    AUTHOR = {Amitsur, S. A. and Rowen, L. H.},
     TITLE = {Elements of reduced trace {$0$}},
   JOURNAL = {Israel J. Math.},
  FJOURNAL = {Israel Journal of Mathematics},
    VOLUME = {87},
      YEAR = {1994},
    NUMBER = {1-3},
     PAGES = {161--179},
      ISSN = {0021-2172},
   MRCLASS = {16K20 (16U99)},
  MRNUMBER = {1286824},
MRREVIEWER = {Patrick J. Morandi},
       DOI = {10.1007/BF02772992},
       URL = {https://doi.org/10.1007/BF02772992},
}

@book {radjavirosenthal,
    AUTHOR = {Radjavi, H. and Rosenthal, P.},
     TITLE = {Simultaneous triangularization},
    SERIES = {Universitext},
 PUBLISHER = {Springer-Verlag, New York},
      YEAR = {2000},
     PAGES = {xii+318},
      ISBN = {0-387-98467-4; 0-387-98466-6},
   MRCLASS = {47-02 (15-02 15A21 47A15 47D03)},
  MRNUMBER = {1736065},
MRREVIEWER = {Donald W. Hadwin},
       DOI = {10.1007/978-1-4612-1200-3},
       URL = {https://doi.org/10.1007/978-1-4612-1200-3},
}

@article{julius2,
  title="On maps preserving {L}ie products equal to e11-e22",
  author={Julius, H.},
  journal={Linear Multilinear Algebra},
  volume={69},
  number={14},
  pages={2620--2628},
  year={2021},
  publisher={Taylor \& Francis}
}

@article{catalanochanglee,
  title={On maps preserving rank-one nilpotents},
  author={Catalano, L. and Chang-Lee, M.},
  journal={Linear Multilinear Algebra},
  volume={69},
  number={16},
  pages={3092--3098},
  year={2021},
  publisher={Taylor \& Francis}
}

@article {amitsurlevitzki,
    AUTHOR = {Amitsur, S. A. and Levitzki, J.},
     TITLE = {Minimal identities for algebras},
   JOURNAL = {Proc. Amer. Math. Soc.},
  FJOURNAL = {Proceedings of the American Mathematical Society},
    VOLUME = {1},
      YEAR = {1950},
     PAGES = {449--463},
      ISSN = {0002-9939},
   MRCLASS = {09.1X},
  MRNUMBER = {36751},
MRREVIEWER = {I. Kaplansky},
       DOI = {10.2307/2032312},
       URL = {https://doi.org/10.2307/2032312},
}

@book {bresarbook,
    AUTHOR = {Bre\v{s}ar, M.},
     TITLE = {Introduction to noncommutative algebra},
    SERIES = {Universitext},
 PUBLISHER = {Springer, Cham},
      YEAR = {2014},
     PAGES = {xxxviii+199},
      ISBN = {978-3-319-08692-7; 978-3-319-08693-4},
   MRCLASS = {16-01},
  MRNUMBER = {3308118},
MRREVIEWER = {Plamen Koshlukov},
       DOI = {10.1007/978-3-319-08693-4},
       URL = {https://doi.org/10.1007/978-3-319-08693-4},
}

@article {wangyou,
    AUTHOR = {Wang, X. T. and You, H.},
     TITLE = {Decomposition of {J}ordan automorphisms of strictly triangular
              matrix algebra over local rings},
   JOURNAL = {Linear Algebra Appl.},
  FJOURNAL = {Linear Algebra and its Applications},
    VOLUME = {392},
      YEAR = {2004},
     PAGES = {183--193},
      ISSN = {0024-3795},
   MRCLASS = {16W20 (16S50 17C99)},
  MRNUMBER = {2095913},
MRREVIEWER = {Santos Gonz\'{a}lez},
       DOI = {10.1016/j.laa.2004.06.009},
       URL = {https://doi.org/10.1016/j.laa.2004.06.009},
}

@article {marcusmoylstensor,
    AUTHOR = {Marcus, M. and Moyls, B. N.},
     TITLE = {Transformations on tensor product spaces},
   JOURNAL = {Pacific J. Math.},
  FJOURNAL = {Pacific Journal of Mathematics},
    VOLUME = {9},
      YEAR = {1959},
     PAGES = {1215--1221},
      ISSN = {0030-8730},
   MRCLASS = {15.00},
  MRNUMBER = {108503},
MRREVIEWER = {L. Mirsky},
       URL = {http://projecteuclid.org/euclid.pjm/1103038893},
}

@article {marcusmoyls,
    AUTHOR = {Marcus, M. and Moyls, B. N.},
     TITLE = {Linear transformations on algebras of matrices},
   JOURNAL = {Canadian J. Math.},
  FJOURNAL = {Canadian Journal of Mathematics. Journal Canadien de
              Math\'{e}matiques},
    VOLUME = {11},
      YEAR = {1959},
     PAGES = {61--66},
      ISSN = {0008-414X},
   MRCLASS = {15.00},
  MRNUMBER = {99996},
MRREVIEWER = {W. E. Jenner},
       DOI = {10.4153/CJM-1959-008-0},
       URL = {https://doi.org/10.4153/CJM-1959-008-0},
}

@article {marcuspurves,
    AUTHOR = {Marcus, M. and Purves, R.},
     TITLE = {Linear transformations on algebras of matrices: the invariance
              of the elementary symmetric functions},
   JOURNAL = {Canadian J. Math.},
  FJOURNAL = {Canadian Journal of Mathematics. Journal Canadien de
              Math\'{e}matiques},
    VOLUME = {11},
      YEAR = {1959},
     PAGES = {383--396},
      ISSN = {0008-414X},
   MRCLASS = {15.00},
  MRNUMBER = {105425},
MRREVIEWER = {L. Mirsky},
       DOI = {10.4153/CJM-1959-039-4},
       URL = {https://doi.org/10.4153/CJM-1959-039-4},
}

@article {jacobsonrickart,
    AUTHOR = {Jacobson, N. and Rickart, C. E.},
     TITLE = {Jordan homomorphisms of rings},
   JOURNAL = {Trans. Amer. Math. Soc.},
  FJOURNAL = {Transactions of the American Mathematical Society},
    VOLUME = {69},
      YEAR = {1950},
     PAGES = {479--502},
      ISSN = {0002-9947},
   MRCLASS = {09.1X},
  MRNUMBER = {38335},
MRREVIEWER = {J. Dieudonn\'{e}},
       DOI = {10.2307/1990495},
       URL = {https://doi.org/10.2307/1990495},
}
	
@article {herstein,
    AUTHOR = {Herstein, I. N.},
     TITLE = {Lie and {J}ordan structures in simple, associative rings},
   JOURNAL = {Bull. Amer. Math. Soc.},
  FJOURNAL = {Bulletin of the American Mathematical Society},
    VOLUME = {67},
      YEAR = {1961},
     PAGES = {517--531},
      ISSN = {0002-9904},
   MRCLASS = {17.60},
  MRNUMBER = {139641},
MRREVIEWER = {E. H. Batho},
       DOI = {10.1090/S0002-9904-1961-10666-6},
       URL = {https://doi.org/10.1090/S0002-9904-1961-10666-6},
}
	
@article {kuzma,
    AUTHOR = {Kuzma, B.},
     TITLE = {Additive mappings preserving rank-one idempotents},
   JOURNAL = {Acta Math. Sin. (Engl. Ser.)},
  FJOURNAL = {Acta Mathematica Sinica (English Series)},
    VOLUME = {21},
      YEAR = {2005},
    NUMBER = {6},
     PAGES = {1399--1406},
      ISSN = {1439-8516},
   MRCLASS = {47B49 (15A04 46B28)},
  MRNUMBER = {2190009},
MRREVIEWER = {Lajos Moln\'{a}r},
       DOI = {10.1007/s10114-005-0598-1},
       URL = {https://doi.org/10.1007/s10114-005-0598-1},
}

@article {jinglilu,
    AUTHOR = {Jing, W. and Li, P. and Lu, S.},
     TITLE = {Additive mappings that preserve rank one nilpotent operators},
   JOURNAL = {Linear Algebra Appl.},
  FJOURNAL = {Linear Algebra and its Applications},
    VOLUME = {367},
      YEAR = {2003},
     PAGES = {213--224},
      ISSN = {0024-3795},
   MRCLASS = {47B49 (47L10)},
  MRNUMBER = {1976920},
MRREVIEWER = {Lajos Moln\'{a}r},
       DOI = {10.1016/S0024-3795(02)00617-1},
       URL = {https://doi.org/10.1016/S0024-3795(02)00617-1},
}

@article {herstein2,
    AUTHOR = {Herstein, I. N.},
     TITLE = {Jordan homomorphisms},
   JOURNAL = {Trans. Amer. Math. Soc.},
  FJOURNAL = {Transactions of the American Mathematical Society},
    VOLUME = {81},
      YEAR = {1956},
     PAGES = {331--341},
      ISSN = {0002-9947},
   MRCLASS = {09.3X},
  MRNUMBER = {76751},
MRREVIEWER = {C. W. Curtis},
       DOI = {10.2307/1992920},
       URL = {https://doi.org/10.2307/1992920},
}

@article {howard,
    AUTHOR = {Howard, R.},
     TITLE = {Linear maps that preserve matrices annihilated by a
              polynomial},
   JOURNAL = {Linear Algebra Appl.},
  FJOURNAL = {Linear Algebra and its Applications},
    VOLUME = {30},
      YEAR = {1980},
     PAGES = {167--176},
      ISSN = {0024-3795},
   MRCLASS = {15A04},
  MRNUMBER = {568789},
MRREVIEWER = {Pl. Kannappan},
       DOI = {10.1016/0024-3795(80)90192-5},
       URL = {https://doi.org/10.1016/0024-3795(80)90192-5},
}

@article {petek,
    AUTHOR = {Petek, T.},
     TITLE = {Mappings preserving the idempotency of products of operators},
   JOURNAL = {Linear Multilinear Algebra},
  FJOURNAL = {Linear and Multilinear Algebra},
    VOLUME = {58},
      YEAR = {2010},
    NUMBER = {7-8},
     PAGES = {903--925},
      ISSN = {0308-1087},
   MRCLASS = {15A86 (47B49)},
  MRNUMBER = {2742325},
MRREVIEWER = {Mikhail Chebotar},
       DOI = {10.1080/03081080903132593},
       URL = {https://doi.org/10.1080/03081080903132593},
}

@article {wangfangli,
    AUTHOR = {Wang, M. and Fang, L. and Ji, G.},
     TITLE = {Linear maps preserving idempotency of products or triple
              {J}ordan products of operators},
   JOURNAL = {Linear Algebra Appl.},
  FJOURNAL = {Linear Algebra and its Applications},
    VOLUME = {429},
      YEAR = {2008},
    NUMBER = {1},
     PAGES = {181--189},
      ISSN = {0024-3795},
   MRCLASS = {47B49},
  MRNUMBER = {2419148},
MRREVIEWER = {Nung-Sing Sze},
       DOI = {10.1016/j.laa.2008.02.013},
       URL = {https://doi.org/10.1016/j.laa.2008.02.013},
}

@article {fangjipang,
    AUTHOR = {Fang, L. and Ji, G. and Pang, Y.},
     TITLE = {Maps preserving the idempotency of products of operators},
   JOURNAL = {Linear Algebra Appl.},
  FJOURNAL = {Linear Algebra and its Applications},
    VOLUME = {426},
      YEAR = {2007},
    NUMBER = {1},
     PAGES = {40--52},
      ISSN = {0024-3795},
   MRCLASS = {47B49},
  MRNUMBER = {2344558},
MRREVIEWER = {Guimei An},
       DOI = {10.1016/j.laa.2007.03.030},
       URL = {https://doi.org/10.1016/j.laa.2007.03.030},
}

@article {gutermanlisemrl,
    AUTHOR = {Guterman, A. and Li, C.-K. and \v{S}emrl, P.},
     TITLE = {Some general techniques on linear preserver problems},
   JOURNAL = {Linear Algebra Appl.},
  FJOURNAL = {Linear Algebra and its Applications},
    VOLUME = {315},
      YEAR = {2000},
    NUMBER = {1-3},
     PAGES = {61--81},
      ISSN = {0024-3795},
   MRCLASS = {15A04 (47B49)},
  MRNUMBER = {1774960},
MRREVIEWER = {Richard D. Hill},
       DOI = {10.1016/S0024-3795(00)00119-1},
       URL = {https://doi.org/10.1016/S0024-3795(00)00119-1},
}
	
@article {lipierce,
    AUTHOR = {Li, C.-K. and Pierce, S.},
     TITLE = {Linear operators preserving similarity classes and related
              results},
   JOURNAL = {Canad. Math. Bull.},
  FJOURNAL = {Canadian Mathematical Bulletin. Bulletin Canadien de
              Math\'{e}matiques},
    VOLUME = {37},
      YEAR = {1994},
    NUMBER = {3},
     PAGES = {374--383},
      ISSN = {0008-4395},
   MRCLASS = {15A69 (15A42)},
  MRNUMBER = {1289774},
MRREVIEWER = {William Watkins},
       DOI = {10.4153/CMB-1994-055-0},
       URL = {https://doi.org/10.4153/CMB-1994-055-0},
}

@article {albertmuckenhoupt,
    AUTHOR = {Albert, A. A. and Muckenhoupt, Benjamin},
     TITLE = {On matrices of trace zeros},
   JOURNAL = {Michigan Math. J.},
  FJOURNAL = {Michigan Mathematical Journal},
    VOLUME = {4},
      YEAR = {1957},
     PAGES = {1--3},
      ISSN = {0026-2285},
   MRCLASS = {15.0X},
  MRNUMBER = {83961},
MRREVIEWER = {D. E. Rutherford},
       URL = {http://projecteuclid.org/euclid.mmj/1028990168},
}

@article {shoda,
    AUTHOR = {Shoda, K.},
     TITLE = {Einige {S}\"{a}tze \"{u}ber {M}atrizen},
   JOURNAL = {Jpn. J. Math.},
  FJOURNAL = {Japanese Journal of Mathematics},
    VOLUME = {13},
      YEAR = {1937},
    NUMBER = {3},
     PAGES = {361--365},
      ISSN = {0075-3432},
   MRCLASS = {15A24},
  MRNUMBER = {3223061},
       DOI = {10.4099/jjm1924.13.0_361},
       URL = {https://doi.org/10.4099/jjm1924.13.0_361},
}

@article{lisemrlsze,
title = "Maps preserving the nilpotency of products of operators",
journal = "Linear Algebra Appl.",
volume = "424",
number = "1",
pages = "222 - 239",
year = "2007",
note = "Special Issue in honor of Roger Horn",
issn = "0024-3795",
doi = "https://doi.org/10.1016/j.laa.2006.11.013",
url = "http://www.sciencedirect.com/science/article/pii/S0024379506005155",
author = "C.-K. Li and Peter Šemrl and Nung-Sing Sze",
keywords = "Preserver, Nilpotent operator, Spectral radius",
}

@article{wong,
author = "Wong, W. J.",
fjournal = "Pacific Journal of Mathematics",
journal = "Pacific J. Math.",
number = "1",
pages = "229--247",
publisher = "Pacific Journal of Mathematics, A Non-profit Corporation",
title = "Maps on simple algebras preserving zero products. {I}. {T}he associative case.",
url = "https://projecteuclid.org:443/euclid.pjm/1102779385",
volume = "89",
year = "1980"
}


@article{gutermankuzma,
author = { A. E.   Guterman  and  B.   Kuzma },
title = {Preserving Zeros of a Polynomial},
journal = {Communications in Algebra},
volume = {37},
number = {11},
pages = {4038-4064},
year  = {2009},
publisher = {Taylor & Francis},
doi = {10.1080/00927870802545687},

URL = { 
        https://doi.org/10.1080/00927870802545687
    
},
eprint = { 
        https://doi.org/10.1080/00927870802545687
    
}

}

@article{linwong,
  title={A note on 2-local maps},
  author={Lin, Y.-F. and Wong, T.-L.},
  journal={Proc. Edinb. Math. Soc.},
  volume={49},
  number={3},
  pages={701--708},
  year={2006},
  publisher={Cambridge University Press}
}

@article{chebotarkeleeshiao, title={On Maps Preserving Products}, volume={48}, DOI={10.4153/CMB-2005-033-8}, number={3}, journal={Canad. Math. Bull.}, publisher={Cambridge University Press}, author={Chebotar, M. A. and Ke, W.-F. and Lee, P.-H. and Shiao, L.-S.}, year={2005}, pages={355–369}}

@article {omladicsemrl,
    AUTHOR = {Omladi\v{c}, M. and \v{S}emrl, P.},
     TITLE = {Additive mappings preserving operators of rank one},
   JOURNAL = {Linear Algebra Appl.},
  FJOURNAL = {Linear Algebra and its Applications},
    VOLUME = {182},
      YEAR = {1993},
     PAGES = {239--256},
      ISSN = {0024-3795},
   MRCLASS = {47B49 (15A99)},
  MRNUMBER = {1207085},
MRREVIEWER = {A. R. Sourour},
       DOI = {10.1016/0024-3795(93)90502-F},
       URL = {https://doi-org.proxy.library.kent.edu/10.1016/0024-3795(93)90502-F},
}

@article {jafariansourour,
    AUTHOR = {Jafarian, A. A. and Sourour, A. R.},
     TITLE = {Spectrum-preserving linear maps},
   JOURNAL = {J. Funct. Anal.},
  FJOURNAL = {Journal of Functional Analysis},
    VOLUME = {66},
      YEAR = {1986},
    NUMBER = {2},
     PAGES = {255--261},
      ISSN = {0022-1236},
   MRCLASS = {47A10 (47D30)},
  MRNUMBER = {832991},
MRREVIEWER = {T. A. Gillespie},
       DOI = {10.1016/0022-1236(86)90073-X},
       URL = {https://doi-org.proxy.library.kent.edu/10.1016/0022-1236(86)90073-X},
}

@book {molnar,
    AUTHOR = {Moln\'{a}r, L.},
     TITLE = {Selected preserver problems on algebraic structures of linear
              operators and on function spaces},
    SERIES = {Lecture Notes in Mathematics},
    VOLUME = {1895},
 PUBLISHER = {Springer-Verlag, Berlin},
      YEAR = {2007},
     PAGES = {xiv+232},
      ISBN = {978-3-540-39944-5; 3-540-39944-5},
   MRCLASS = {47B49 (46J10 47L05 47N50 81R15)},
  MRNUMBER = {2267033},
MRREVIEWER = {Matej Bre\v{s}ar},
}

@article {pankov,
    AUTHOR = {Pankov, M.},
     TITLE = {Wigner's type theorem in terms of linear operators which send
              projections of a fixed rank to projections of other fixed
              rank},
   JOURNAL = {J. Math. Anal. Appl.},
  FJOURNAL = {Journal of Mathematical Analysis and Applications},
    VOLUME = {474},
      YEAR = {2019},
    NUMBER = {2},
     PAGES = {1238--1249},
      ISSN = {0022-247X},
   MRCLASS = {81P16 (47A46)},
  MRNUMBER = {3926164},
       DOI = {10.1016/j.jmaa.2019.02.014},
       URL = {https://doi.org/10.1016/j.jmaa.2019.02.014},
}

@article {bresarsemrl3,
    AUTHOR = {Bre\v{s}ar, M. and \v{S}emrl, P.},
     TITLE = {On local automorphisms and mappings that preserve idempotents},
   JOURNAL = {Studia Math.},
  FJOURNAL = {Studia Mathematica},
    VOLUME = {113},
      YEAR = {1995},
    NUMBER = {2},
     PAGES = {101--108},
      ISSN = {0039-3223},
   MRCLASS = {47B48 (46L40 47D99)},
  MRNUMBER = {1318418},
       DOI = {10.4064/sm-113-2-101-108},
       URL = {https://doi-org.proxy.library.kent.edu/10.4064/sm-113-2-101-108},
}
	
	@article {semrlidem,
    AUTHOR = {\v{S}emrl, P.},
     TITLE = {Applying projective geometry to transformations on rank one
              idempotents},
   JOURNAL = {J. Funct. Anal.},
  FJOURNAL = {Journal of Functional Analysis},
    VOLUME = {210},
      YEAR = {2004},
    NUMBER = {1},
     PAGES = {248--257},
      ISSN = {0022-1236},
   MRCLASS = {47B49},
  MRNUMBER = {2052121},
MRREVIEWER = {Jor-Ting Chan},
       DOI = {10.1016/j.jfa.2003.07.009},
       URL = {https://doi-org.proxy.library.kent.edu/10.1016/j.jfa.2003.07.009},
}

@article {wangwu,
    AUTHOR = {Wang, J.-H. and Wu, P.-Y.},
     TITLE = {Sums of square-zero operators},
   JOURNAL = {Studia Math.},
  FJOURNAL = {Polska Akademia Nauk. Instytut Matematyczny. Studia
              Mathematica},
    VOLUME = {99},
      YEAR = {1991},
    NUMBER = {2},
     PAGES = {115--127},
      ISSN = {0039-3223},
   MRCLASS = {47B99 (15A99 47A99 47B47)},
  MRNUMBER = {1120744},
MRREVIEWER = {A. R. Sourour},
       DOI = {10.4064/sm-99-2-115-127},
       URL = {https://doi-org.proxy.library.kent.edu/10.4064/sm-99-2-115-127},
}

@article {fillmore,
    AUTHOR = {Fillmore, P. A.},
     TITLE = {Sums of operators with square zero},
   JOURNAL = {Acta Sci. Math. (Szeged)},
  FJOURNAL = {Acta Universitatis Szegediensis. Acta Scientiarum
              Mathematicarum},
    VOLUME = {28},
      YEAR = {1967},
     PAGES = {285--288},
      ISSN = {0001-6969},
   MRCLASS = {47.10},
  MRNUMBER = {221301},
MRREVIEWER = {C. R. Putnam},
}
			
@article {geher,
    AUTHOR = {Geh\'{e}r, Gy. P.},
     TITLE = {Wigner's theorem on {G}rassmann spaces},
   JOURNAL = {J. Funct. Anal.},
  FJOURNAL = {Journal of Functional Analysis},
    VOLUME = {273},
      YEAR = {2017},
    NUMBER = {9},
     PAGES = {2994--3001},
      ISSN = {0022-1236},
   MRCLASS = {47C05 (81P10 81Q12 81R15)},
  MRNUMBER = {3692328},
MRREVIEWER = {Alexander Isaakovich Shtern},
       DOI = {10.1016/j.jfa.2017.06.011},
       URL = {https://doi-org.proxy.library.kent.edu/10.1016/j.jfa.2017.06.011},
}

@article{BCSP,
  title={Linear maps between {C}*-algebras that are *-homomorphisms at a fixed point},
  author={Burgos, M. J and S{\'a}nchez, J. C. and Peralta, A. M.},
  journal={Quaestiones Mathematicae},
  volume={42},
  number={2},
  pages={151--164},
  year={2019},
  publisher={Taylor \& Francis}
}

@article{eidelheit,
  title={On isomorphisms of rings of linear operators},
  author={Eidelheit, M.},
  journal={Studia Math.},
  volume={9},
  pages={97--105},
  year={1940},
  publisher={Instytut Matematyczny Polskiej Akademii Nauk}
}

@article {sharmaalmeida,
    AUTHOR = {Sharma, C. S. and Almeida, D. F.},
     TITLE = {A direct proof of {W}igner's theorem on maps which preserve
              transition probabilities between pure states of quantum
              systems},
   JOURNAL = {Ann. Physics},
  FJOURNAL = {Annals of Physics},
    VOLUME = {197},
      YEAR = {1990},
    NUMBER = {2},
     PAGES = {300--309},
      ISSN = {0003-4916},
   MRCLASS = {81P05 (46N50 47A99)},
  MRNUMBER = {1036085},
MRREVIEWER = {S. D. Chatterji},
       DOI = {10.1016/0003-4916(90)90213-8},
       URL = {https://doi-org.proxy.library.kent.edu/10.1016/0003-4916(90)90213-8},
}

@article{catalano,
author = {L. Catalano},
title = {On maps preserving products equal to a rank-one idempotent},
journal = {Linear Multilinear Algebra},
volume = {0},
number = {0},
pages = {1-8},
year  = {2019},
publisher = {Taylor & Francis},
doi = {10.1080/03081087.2019.1614518},

URL = { 
        https://doi.org/10.1080/03081087.2019.1614518
    
},
eprint = { 
        https://doi.org/10.1080/03081087.2019.1614518
    
}
}

@article {bresarzpd,
    AUTHOR = {Bre\v{s}ar, M. and Gra\v{s}i\v{c}, M. and Ortega, J. S\'{a}nchez},
     TITLE = {Zero product determined matrix algebras},
   JOURNAL = {Linear Algebra Appl.},
  FJOURNAL = {Linear Algebra and its Applications},
    VOLUME = {430},
      YEAR = {2009},
    NUMBER = {5-6},
     PAGES = {1486--1498},
      ISSN = {0024-3795},
   MRCLASS = {16S50 (16W10)},
  MRNUMBER = {2490691},
MRREVIEWER = {J\"{u}rgen M\"{u}ller},
       DOI = {10.1016/j.laa.2007.11.018},
       URL = {https://doi-org.proxy.library.kent.edu/10.1016/j.laa.2007.11.018},
}

@article {grasic,
    AUTHOR = {Gra\v{s}i\v{c}, M.},
     TITLE = {Zero product determined classical {L}ie algebras},
   JOURNAL = {Linear Multilinear Algebra},
  FJOURNAL = {Linear and Multilinear Algebra},
    VOLUME = {58},
      YEAR = {2010},
    NUMBER = {7-8},
     PAGES = {1007--1022},
      ISSN = {0308-1087},
   MRCLASS = {17B20 (15A27)},
  MRNUMBER = {2742332},
MRREVIEWER = {Francesco Regonati},
       DOI = {10.1080/03081080903191672},
       URL = {https://doi-org.proxy.library.kent.edu/10.1080/03081080903191672},
}
	
@book {bresarzpdbook,
    AUTHOR = {Bre\v{s}ar, M.},
     TITLE = {Zero product determined algebras},
    SERIES = {Frontiers in Mathematics},
 PUBLISHER = {Birkh\"{a}user/Springer, Cham},
      YEAR = {2021},
     PAGES = {185},
      ISBN = {978-3-030-80241-7; 978-3-030-80242-4},
   MRCLASS = {16W25 (16W20 17A01 46H70 47B47 47B49)},
  MRNUMBER = {4311188},
       DOI = {10.1007/978-3-030-80242-4},
       URL = {https://doi-org.proxy.library.kent.edu/10.1007/978-3-030-80242-4},
}
	
	
	
@article {bresarzpd2,
    AUTHOR = {Bre\v{s}ar, M.},
     TITLE = {Finite dimensional zero product determined algebras are
              generated by idempotents},
   JOURNAL = {Expo. Math.},
  FJOURNAL = {Expositiones Mathematicae},
    VOLUME = {34},
      YEAR = {2016},
    NUMBER = {1},
     PAGES = {130--143},
      ISSN = {0723-0869},
   MRCLASS = {16P10 (16K20)},
  MRNUMBER = {3463687},
MRREVIEWER = {Hoger Ghahramani},
       DOI = {10.1016/j.exmath.2015.07.002},
       URL = {https://doi-org.proxy.library.kent.edu/10.1016/j.exmath.2015.07.002},
}

@article {semrlaut,
    AUTHOR = {\v{S}emrl, P.},
     TITLE = {Automorphisms of {H}ilbert space effect algebras},
   JOURNAL = {J. Phys. A},
  FJOURNAL = {Journal of Physics. A. Mathematical and Theoretical},
    VOLUME = {48},
      YEAR = {2015},
    NUMBER = {19},
     PAGES = {195301, 18},
      ISSN = {1751-8113},
   MRCLASS = {47A05 (46C15)},
  MRNUMBER = {3342767},
MRREVIEWER = {Toka Diagana},
       DOI = {10.1088/1751-8113/48/19/195301},
       URL = {https://doi-org.proxy.library.kent.edu/10.1088/1751-8113/48/19/195301},
}

@article {semrlsym,
    AUTHOR = {\v{S}emrl, P.},
     TITLE = {Symmetries of {H}ilbert space effect algebras},
   JOURNAL = {J. Lond. Math. Soc. (2)},
  FJOURNAL = {Journal of the London Mathematical Society. Second Series},
    VOLUME = {88},
      YEAR = {2013},
    NUMBER = {2},
     PAGES = {417--436},
      ISSN = {0024-6107},
   MRCLASS = {47B49 (81P15)},
  MRNUMBER = {3106729},
MRREVIEWER = {Tatjana Petek},
       DOI = {10.1112/jlms/jdt021},
       URL = {https://doi-org.proxy.library.kent.edu/10.1112/jlms/jdt021},
}

@article {LTW,
    AUTHOR = {Li, C.-K. and Tsai, M.-C. and Wang, Y.-S and Wong,
              N.-C.},
     TITLE = {Nonsurjective maps between rectangular matrix spaces
              preserving disjointness, triple products, or norms},
   JOURNAL = {J. Operator Theory},
  FJOURNAL = {Journal of Operator Theory},
    VOLUME = {83},
      YEAR = {2020},
    NUMBER = {1},
     PAGES = {27--53},
      ISSN = {0379-4024},
   MRCLASS = {15A86 (15A04 15A60 47B49)},
  MRNUMBER = {4043705},
MRREVIEWER = {Wai Shun Cheung},
       DOI = {10.7900/jot},
       URL = {https://doi-org.proxy.library.kent.edu/10.7900/jot},
}

@article {LRS,
    AUTHOR = {Li, C.-K. and Rodman, L. and \v{S}emrl, P.},
     TITLE = {Linear transformations between matrix spaces that map one rank
              specific set into another},
   JOURNAL = {Linear Algebra Appl.},
  FJOURNAL = {Linear Algebra and its Applications},
    VOLUME = {357},
      YEAR = {2002},
     PAGES = {197--208},
      ISSN = {0024-3795},
   MRCLASS = {15A04 (15A03)},
  MRNUMBER = {1935234},
MRREVIEWER = {Donald W. Robinson},
       DOI = {10.1016/S0024-3795(02)00381-6},
       URL = {https://doi-org.proxy.library.kent.edu/10.1016/S0024-3795(02)00381-6},
}

@article {LTWW,
    AUTHOR = {Li, C.-K. and Tsai, M.-C. and Wang, Y.-S. and Wong,
              N.-C.},
     TITLE = {Nonsurjective maps between rectangular matrix spaces
              preserving disjointness, triple products, or norms},
   JOURNAL = {J. Operator Theory},
  FJOURNAL = {Journal of Operator Theory},
    VOLUME = {83},
      YEAR = {2020},
    NUMBER = {1},
     PAGES = {27--53},
      ISSN = {0379-4024},
   MRCLASS = {15A86 (15A04 15A60 47B49)},
  MRNUMBER = {4043705},
MRREVIEWER = {Wai Shun Cheung},
       DOI = {10.7900/jot},
       URL = {https://doi-org.proxy.library.kent.edu/10.7900/jot},
}

@article {sinkhorn,
    AUTHOR = {Sinkhorn, R.},
     TITLE = {Linear adjugate preservers on the complex matrices},
   JOURNAL = {Linear Multilinear Algebra},
  FJOURNAL = {Linear and Multilinear Algebra},
    VOLUME = {12},
      YEAR = {1982/83},
    NUMBER = {3},
     PAGES = {215--222},
      ISSN = {0308-1087},
   MRCLASS = {15A04},
  MRNUMBER = {678827},
MRREVIEWER = {W. Ledermann},
       DOI = {10.1080/03081088208817485},
       URL = {https://doi-org.proxy.library.kent.edu/10.1080/03081088208817485},

}

@article{houcui,
  title={Additive maps on standard operator algebras preserving invertibilities or zero divisors},
  author={Hou, J. and Cui, J.},
  journal={Linear Algebra Appl.},
  volume={359},
  number={1-3},
  pages={219--233},
  year={2003},
  publisher={Elsevier}
}

@article{zhaohou,
  title={Jordan zero-product preserving additive maps on operator algebras},
  author={Zhao, L. and Hou, J.},
  journal={J. Math. Anal. Appl.},
  volume={314},
  number={2},
  pages={689--700},
  year={2006},
  publisher={Elsevier}
}

@book{frobenius,
  title={{\"U}ber die Darstellung der endlichen Gruppen durch lineare Substitutionen},
  author={Frobenius, G.},
  year={1897},
  publisher={Reichsdr.}
}

@article{BJS,
AUTHOR = {Borisov, N. and Julius, H. and Sikora, M.},
TITLE = {On maps preserving square roots of idempotent and rank-one nilpotent matrices},
JOURNAL = {J. Algebra Appl.},
FJOURNAL = {Journal of Algebra and its Applications.},
YEAR = {2021},
NOTE = {To Appear.},
}

@article{catalanojulius,
  title={On maps preserving products equal to fixed elements},
  author={Catalano, L. and Julius, H.},
  journal={J. Algebra},
  fjournal={Journal of Algebra},
  volume={575},
  pages={220--232},
  year={2021},
  publisher={Elsevier}
}

@article{zhu,
  title={Multiplicative mappings at some points on matrix algebras},
  author={Zhu, J. and Xiong, C. and Zhu, H.},
  journal={Linear Algebra Appl.},
  volume={433},
  number={5},
  pages={914--927},
  year={2010},
  publisher={Elsevier}
}

@article{catalanojulius2,
author = {L. Catalano and H. Julius},
title = {On maps preserving products equal to a diagonalizable matrix},
journal = {Comm. Algebra},
volume = {49},
number = {10},
pages = {4334-4344},
year  = {2021},
publisher = {Taylor & Francis},
doi = {10.1080/00927872.2021.1919133},

URL = { 
        https://doi.org/10.1080/00927872.2021.1919133
    
},
eprint = { 
        https://doi.org/10.1080/00927872.2021.1919133
    
}

}

@article {keliwong,
    AUTHOR = {Ke, W.-F. and Li, B.-R. and Wong, N.-C.},
     TITLE = {Zero product preserving maps of operator-valued functions},
   JOURNAL = {Proc. Amer. Math. Soc.},
  FJOURNAL = {Proceedings of the American Mathematical Society},
    VOLUME = {132},
      YEAR = {2004},
    NUMBER = {7},
     PAGES = {1979--1985},
      ISSN = {0002-9939},
   MRCLASS = {47B48 (46E40 46H05 47B33)},
  MRNUMBER = {2053969},
MRREVIEWER = {Jesus Araujo},
       DOI = {10.1090/S0002-9939-03-07321-0},
       URL = {https://doi-org.proxy.library.kent.edu/10.1090/S0002-9939-03-07321-0},
}

@article {ke2,
    AUTHOR = {Chebotar, M. A. and Ke, W.-F. and Lee, P.-H. and Shiao, L.-S.},
     TITLE = {On maps preserving products},
   JOURNAL = {Canad. Math. Bull.},
  FJOURNAL = {Canadian Mathematical Bulletin. Bulletin Canadien de
              Math\'{e}matiques},
    VOLUME = {48},
      YEAR = {2005},
    NUMBER = {3},
     PAGES = {355--369},
      ISSN = {0008-4395},
   MRCLASS = {16S99 (16W20 17B40)},
  MRNUMBER = {2154078},
MRREVIEWER = {Celestina Cotti-Ferrero},
       DOI = {10.4153/CMB-2005-033-8},
       URL = {https://doi-org.proxy.library.kent.edu/10.4153/CMB-2005-033-8},
}

@article {ke3,
    AUTHOR = {Chebotar, M. A. and Ke, W.-F. and Lee, P.-H.},
     TITLE = {On maps preserving square-zero matrices},
   JOURNAL = {J. Algebra},
  FJOURNAL = {Journal of Algebra},
    VOLUME = {289},
      YEAR = {2005},
    NUMBER = {2},
     PAGES = {421--445},
      ISSN = {0021-8693},
   MRCLASS = {16S50 (16R99)},
  MRNUMBER = {2142380},
MRREVIEWER = {Pedro A. Guil Asensio},
       DOI = {10.1016/j.jalgebra.2005.01.018},
       URL = {https://doi-org.proxy.library.kent.edu/10.1016/j.jalgebra.2005.01.018},
}

@article {ke4,
    AUTHOR = {Chebotar, M. A. and Ke, W.-F. and Lee, P.-H.},
     TITLE = {Maps preserving zero {J}ordan products on {H}ermitian
              operators},
   JOURNAL = {Illinois J. Math.},
  FJOURNAL = {Illinois Journal of Mathematics},
    VOLUME = {49},
      YEAR = {2005},
    NUMBER = {2},
     PAGES = {445--452},
      ISSN = {0019-2082},
   MRCLASS = {47B48 (16W10 17C30 46L70)},
  MRNUMBER = {2164345},
MRREVIEWER = {Borut Zalar},
       URL = {http://projecteuclid.org.proxy.library.kent.edu/euclid.ijm/1258138027},
}

@article {dixon,
    AUTHOR = {Dixon, J. D.},
     TITLE = {Rigid embedding of simple groups in the general linear group},
   JOURNAL = {Canadian J. Math.},
  FJOURNAL = {Canadian Journal of Mathematics. Journal Canadien de
              Math\'{e}matiques},
    VOLUME = {29},
      YEAR = {1977},
    NUMBER = {2},
     PAGES = {384--391},
      ISSN = {0008-414X},
   MRCLASS = {20G20},
  MRNUMBER = {435242},
MRREVIEWER = {David Birkes},
       DOI = {10.4153/CJM-1977-041-0},
       URL = {https://doi-org.proxy.library.kent.edu/10.4153/CJM-1977-041-0},
}

@book {baer,
    AUTHOR = {Baer, R.},
     TITLE = {Linear algebra and projective geometry},
 PUBLISHER = {Academic Press Inc., New York, N. Y.},
      YEAR = {1952},
     PAGES = {viii+318},
   MRCLASS = {48.0X},
  MRNUMBER = {0052795},
MRREVIEWER = {F. W. Levi},
}

@article{molnarsemrl,
author = {L. Molnár  and  P. \v{S}emrl },
title = {Some linear preserver problems on upper triangular matrices},
journal = {Linear Multilinear Algebra},
volume = {45},
number = {2-3},
pages = {189-206},
year  = {1998},
publisher = {Taylor & Francis},
doi = {10.1080/03081089808818586},

URL = { 
        https://doi.org/10.1080/03081089808818586
    
},
eprint = { 
        https://doi.org/10.1080/03081089808818586
    
}

}
@article {hua,
    AUTHOR = {Hua, L.-K.},
     TITLE = {A theorem on matrices over a sfield and its applications},
   JOURNAL = {J. Chinese Math. Soc. (N.S.)},
    VOLUME = {1},
      YEAR = {1951},
     PAGES = {110--163},
   MRCLASS = {09.3X},
  MRNUMBER = {0071414},
MRREVIEWER = {J. Dieudonn\'{e}},
}

@article{boudimbekhta,
 ISSN = {03794024, 18417744},
 URL = {http://www.jstor.org/stable/24715945},
 author = {N. Boudi and M. Mbekhta},
 journal = {J. Operator Theory},
 number = {1},
 pages = {117--130},
 publisher = {Theta Foundation},
 title = {ADDITIVE MAPS PRESERVING STRONGLY GENERALIZED INVERSES},
 volume = {64},
 year = {2010}
}



@article {EK,
    AUTHOR = {Essannouni, H. and Kaidi, A.},
     TITLE = {Le th\'{e}or\`eme de {H}ua pour les alg\`ebres artiniennes simples},
   JOURNAL = {Linear Algebra Appl.},
  FJOURNAL = {Linear Algebra and its Applications},
    VOLUME = {297},
      YEAR = {1999},
    NUMBER = {1-3},
     PAGES = {9--22},
      ISSN = {0024-3795},
   MRCLASS = {16K20 (16W10)},
  MRNUMBER = {1723834},
MRREVIEWER = {W. D. Burgess},
       DOI = {10.1016/S0024-3795(99)00081-6},
       URL = {https://doi-org.proxy.library.kent.edu/10.1016/S0024-3795(99)00081-6},
}

@article {chanlim,
    AUTHOR = {Chan, G.-H. and Lim, M.-H.},
     TITLE = {Linear preservers on powers of matrices},
      NOTE = {Directions in matrix theory (Auburn, AL, 1990)},
   JOURNAL = {Linear Algebra Appl.},
  FJOURNAL = {Linear Algebra and its Applications},
    VOLUME = {162/164},
      YEAR = {1992},
     PAGES = {615--626},
      ISSN = {0024-3795},
   MRCLASS = {15A04 (15A57)},
  MRNUMBER = {1148420},
MRREVIEWER = {Chi-Kwong Li},
       DOI = {10.1016/0024-3795(92)90396-R},
       URL = {https://doi-org.proxy.library.kent.edu/10.1016/0024-3795(92)90396-R},
}
		
@article {bresarcentralizers,
    AUTHOR = {Bre\v{s}ar, M.},
     TITLE = {Algebras in which non-scalar elements have small centralizers},
   JOURNAL = {Linear Multilinear Algebra},
  FJOURNAL = {Linear and Multilinear Algebra},
    VOLUME = {63},
      YEAR = {2015},
    NUMBER = {9},
     PAGES = {1864--1871},
      ISSN = {0308-1087},
   MRCLASS = {16K20 (15A27 15A78 16N40 16P10)},
  MRNUMBER = {3305015},
MRREVIEWER = {Iuliu Crivei},
       DOI = {10.1080/03081087.2014.977842},
       URL = {https://doi-org.proxy.library.kent.edu/10.1080/03081087.2014.977842},
}

@article {cklz,
    AUTHOR = {Chebotar, M. A. and Ke, W.-F. and Lee, P.-H. and
              Zhang, R.},
     TITLE = {On maps preserving zero {J}ordan products},
   JOURNAL = {Monatsh. Math.},
  FJOURNAL = {Monatshefte f\"{u}r Mathematik},
    VOLUME = {149},
      YEAR = {2006},
    NUMBER = {2},
     PAGES = {91--101},
      ISSN = {0026-9255},
   MRCLASS = {47B49 (15A04)},
  MRNUMBER = {2264576},
MRREVIEWER = {Matej Bre\v{s}ar},
       DOI = {10.1007/s00605-005-0371-7},
       URL = {https://doi-org.proxy.library.kent.edu/10.1007/s00605-005-0371-7},
}

@article{omladicradjavisemrl,
title = {Preserving commutativity},
journal = {Journal of Pure and Applied Algebra},
volume = {156},
number = {2},
pages = {309-328},
year = {2001},
issn = {0022-4049},
doi = {https://doi.org/10.1016/S0022-4049(99)00154-1},
url = {https://www.sciencedirect.com/science/article/pii/S0022404999001541},
author = {M. Omladi\v{c} and H. Radjavi and P. \v{S}emrl},
abstract = {Every commutativity preserving linear map on the algebra of all n×n matrices over an algebraically closed field F with characteristic 0 is either a Jordan automorphism multiplied by a nonzero constant and perturbed by a scalar type operator, or its image is commutative. The assumption of preserving commutativity can be reformulated as preserving zero Lie products. So, this theorem is an extension of the well-known result on the structure of Lie homomorphisms of matrix algebras. We first prove the result for the special case in which F is the complex field and then apply the transfer principle in Model Theoretic Algebra to extend it to the general case.}
}

@article {mirzakhani,
    AUTHOR = {Mirzakhani, M.},
     TITLE = {A simple proof of a theorem of {S}chur},
   JOURNAL = {Amer. Math. Monthly},
  FJOURNAL = {American Mathematical Monthly},
    VOLUME = {105},
      YEAR = {1998},
    NUMBER = {3},
     PAGES = {260--262},
      ISSN = {0002-9890},
   MRCLASS = {15A27},
  MRNUMBER = {1615548},
       DOI = {10.2307/2589084},
       URL = {https://doi-org.proxy.library.kent.edu/10.2307/2589084},
}

@article {wongII,
    AUTHOR = {Wong, W. J.},
     TITLE = {Maps on simple algebras preserving zero products. {II}. {L}ie
              algebras of linear type},
   JOURNAL = {Pacific J. Math.},
  FJOURNAL = {Pacific Journal of Mathematics},
    VOLUME = {92},
      YEAR = {1981},
    NUMBER = {2},
     PAGES = {469--488},
      ISSN = {0030-8730},
   MRCLASS = {15A04 (16A46 17B60)},
  MRNUMBER = {618078},
MRREVIEWER = {L. M. Chawla},
       URL = {http://projecteuclid.org.proxy.library.kent.edu/euclid.pjm/1102736805},
}

@article {laffeyloewy,
    AUTHOR = {Laffey, T. J. and Loewy, R.},
     TITLE = {Linear transformations which do not increase rank},
   JOURNAL = {Linear Multilinear Algebra},
  FJOURNAL = {Linear and Multilinear Algebra},
    VOLUME = {26},
      YEAR = {1990},
    NUMBER = {3},
     PAGES = {181--186},
      ISSN = {0308-1087},
   MRCLASS = {15A04},
  MRNUMBER = {1040780},
MRREVIEWER = {Larry Basen\v{s}piler},
       DOI = {10.1080/03081089008817974},
       URL = {https://doi-org.proxy.library.kent.edu/10.1080/03081089008817974},
}

@article {dieudonne,
    AUTHOR = {Dieudonn\'{e}, Jean},
     TITLE = {Sur une g\'{e}n\'{e}ralisation du groupe orthogonal \`a quatre
              variables},
   JOURNAL = {Arch. Math.},
  FJOURNAL = {Archiv der Mathematik},
    VOLUME = {1},
      YEAR = {1949},
     PAGES = {282--287},
      ISSN = {0003-889X},
   MRCLASS = {09.0X},
  MRNUMBER = {29360},
MRREVIEWER = {L. K. Hua},
       DOI = {10.1007/BF02038756},
       URL = {https://doi-org.proxy.library.kent.edu/10.1007/BF02038756},
}

@article{tarcsay,
title = {Maps preserving the Douglas solution of operator equations},
journal = {J. Math. Anal. and Appl.},
volume = {507},
number = {2},
pages = {125802},
year = {2022},
issn = {0022-247X},
doi = {https://doi.org/10.1016/j.jmaa.2021.125802},
url = {https://www.sciencedirect.com/science/article/pii/S0022247X21008817},
author = {Zsigmond Tarcsay},
keywords = {Douglas theorem, Operator equation, Preserver problem},
abstract = {We consider bijective maps ϕ on the full operator algebra B(H) of an infinite dimensional Hilbert space with the property that, for every A,B,X∈B(H), X is the Douglas solution of the equation A=BX if and only if Y=ϕ(X) is the Douglas solution of the equation ϕ(A)=ϕ(B)Y. We prove that those maps are implemented by a unitary or anti-unitary map U, i.e., ϕ(A)=UAU⁎.}
}

@article {costara,
    AUTHOR = {Costara, C.},
     TITLE = {Nonlinear invertibility preserving maps on matrix algebras},
   JOURNAL = {Linear Algebra Appl.},
  FJOURNAL = {Linear Algebra and its Applications},
    VOLUME = {602},
      YEAR = {2020},
     PAGES = {216--222},
      ISSN = {0024-3795},
   MRCLASS = {15A15 (15A86)},
  MRNUMBER = {4102781},
MRREVIEWER = {Jor-Ting Chan},
       DOI = {10.1016/j.laa.2020.05.010},
       URL = {https://doi.org/10.1016/j.laa.2020.05.010},
}

@article {costara2,
    AUTHOR = {Costara, C.},
     TITLE = {Nonlinear commuting maps on {$\mathcal L(X)$}},
   JOURNAL = {Linear Multilinear Algebra},
  FJOURNAL = {Linear and Multilinear Algebra},
    VOLUME = {69},
      YEAR = {2021},
    NUMBER = {3},
     PAGES = {551--556},
      ISSN = {0308-1087},
   MRCLASS = {47B49 (47B47)},
  MRNUMBER = {4220670},
       DOI = {10.1080/03081087.2019.1607819},
       URL = {https://doi.org/10.1080/03081087.2019.1607819},
}

@article {dolinarsemrl,
    AUTHOR = {Dolinar, G. and \v{S}emrl, P.},
     TITLE = {Determinant preserving maps on matrix algebras},
   JOURNAL = {Linear Algebra Appl.},
  FJOURNAL = {Linear Algebra and its Applications},
    VOLUME = {348},
      YEAR = {2002},
     PAGES = {189--192},
      ISSN = {0024-3795},
   MRCLASS = {15A15},
  MRNUMBER = {1902124},
       DOI = {10.1016/S0024-3795(01)00578-X},
       URL = {https://doi.org/10.1016/S0024-3795(01)00578-X},
}

@article {dolinar,
    AUTHOR = {Dolinar, G.},
     TITLE = {Maps on {$M_n$} preserving {L}ie products},
   JOURNAL = {Publ. Math. Debrecen},
  FJOURNAL = {Publicationes Mathematicae Debrecen},
    VOLUME = {71},
      YEAR = {2007},
    NUMBER = {3-4},
     PAGES = {467--477},
      ISSN = {0033-3883},
   MRCLASS = {17B60 (15A04 17B40)},
  MRNUMBER = {2361725},
MRREVIEWER = {Vesselin Drensky},
}

@article {semrlnonlinear,
    AUTHOR = {\v{S}emrl, P.},
     TITLE = {Non-linear commutativity preserving maps},
   JOURNAL = {Acta Sci. Math. (Szeged)},
  FJOURNAL = {Acta Universitatis Szegediensis. Acta Scientiarum
              Mathematicarum},
    VOLUME = {71},
      YEAR = {2005},
    NUMBER = {3-4},
     PAGES = {781--819},
      ISSN = {0001-6969},
   MRCLASS = {47B49 (15A30 51A05)},
  MRNUMBER = {2206609},
MRREVIEWER = {Chi-Kwong Li},
}
